RPN 2: On Interdependence Function Learning Towards Unifying and Advancing CNN, RNN, GNN, and Transformer

This paper builds upon our previous work on the Reconciled Polynomial Network (RPN). The original RPN model was designed under the assumption of input data independence, presuming the independence among both individual instances within data batches and attributes in each data instance. However, this assumption often proves invalid for function learning tasks involving complex, interdependent data such as language, images, time series, and graphs. Ignoring such data interdependence may inevitably lead to significant performance degradation. To overcome these limitations, we introduce the new Reconciled Polynomial Network (version 2), namely RPN 2, in this paper. By incorporating data and structural interdependence functions, RPN 2 explicitly models data interdependence via new component functions in its architecture. This enhancement not only significantly improves RPN 2's learning performance but also substantially expands its unifying potential, enabling it to encompass a broader range of contemporary dominant backbone models within its canonical representation. These backbones include, but are not limited to, convolutional neural networks (CNNs), recurrent neural networks (RNNs), graph neural networks (GNNs), and Transformers. Our analysis reveals that the fundamental distinctions among these backbone models primarily stem from their diverse approaches to defining the interdependence functions. Furthermore, this unified representation opens up new opportunities for designing innovative architectures with the potential to surpass the performance of these dominant backbones.

==> sections/sec_function_diagram_3.tex <==
%------------------------------------------------------------------------------------
%\vspace{2em}
%\hrule
\begin{figure*}[t]
    \begin{center}
    \tiny
            \begin{forest}
                for tree={
                    forked edges,
                    grow'=0,
                    s sep=2.1pt,
                    draw,
                    rounded corners,
                    node options={align=center,},
                    text width=2.7cm,
                },
                %[\rotatebox{90}{\textcolor{Plum}{\textbf{Reconciled Polynomial Network ({\our})}}}, fill=Plum!30, parent
                [{\textcolor{Plum}{\textbf{Reconciled\\ Polynomial\\ Network\\ ({\our})}}}, fill=Plum!30, parent
                %------------------------------------------------------------
                	    [Data\\ Compression\\ Functions, for tree={fill=brown!45, child}
                    	%-------------------------------------------------------------
                    	[1. Hermite Expansion, fill=brown!30, grandchild
                    		[{1-(a). $\kappa(\mb{x} | d)  = \left[ He_1(\mb{x}), He_2(\mb{x}), \cdots, He_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[2. Laguerre Expansion, fill=brown!30, grandchild
                    		[{2-(a). $\kappa(\mb{x} | d, \alpha) = \left[ P^{(\alpha)}_1(\mb{x}), P^{(\alpha)}_2(\mb{x}), \cdots, P^{(\alpha)}_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[3. Legendre Expansion, fill=brown!30, grandchild
                    		[{3-(a). $\kappa(\mb{x} | d) = \left[ P_1(\mb{x}), P_2(\mb{x}), \cdots, P_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[4. Gegenbauer Expansion, fill=brown!30, grandchild
                    		[{4-(a). $\kappa(\mb{x} | d, \alpha) = \left[ P^{(\alpha)}_1(\mb{x}), P^{(\alpha)}_2(\mb{x}), \cdots, P^{(\alpha)}_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[5. Bessel Expansion, fill=brown!30, grandchild
                    		[{5-(a). $\kappa(\mb{x} | d) = \left[ B_1(\mb{x}), B_2(\mb{x}), \cdots, B_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
				[{5-(b). $\kappa(\mb{x} | d) = \left[ R_1(\mb{x}), R_2(\mb{x}), \cdots, R_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[6. Fibonacci Expansion, fill=brown!30, grandchild
                    		[{6-(a). $\kappa(\mb{x} | d) = \left[ F_1(\mb{x}), F_2(\mb{x}), \cdots, F_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[7. Lucas Expansion, fill=brown!30, grandchild
                    		[{7-(a). $\kappa(\mb{x} | d) = \left[ L_1(\mb{x}), L_2(\mb{x}), \cdots, L_d(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=md$}, fill=brown!15, referenceblock]
                            	]
                        ]
                        %-------------------------------------------------------------
                    	[8. Lucas Expansion, fill=brown!30, grandchild
                    		[{8-(a). $\kappa(\mb{x} | d=1) = \left[ \phi_{0, 0}(\mb{x}), \phi_{0, 1}(\mb{x}), \cdots, \phi_{s, t}(\mb{x}) \right]$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=s \cdot t \cdot m$}, fill=brown!15, referenceblock]
                            	]
				[{8-(b). $\kappa(\mb{x} | d=2) = \kappa(\mb{x} | d=1) \otimes \kappa(\mb{x} | d=1)$}, fill=brown!30, greatgrandchild
                                		[dim: {$D=(s \cdot t \cdot m)^2$}, fill=brown!15, referenceblock]
                            	]
                        ]
                    ]                    
                    [Parameter Reconciliation\\ Functions, for tree={fill=red!45,child}
                    	%-------------------------------------------------------------
                    	[1. Random Matrix Adaption based Reconciliation, fill=red!30, grandchild
				[{1-(a). $\psi(\mb{w}) = \bs{\Lambda}_1 \mb{A} \bs{\Lambda}_1 \mb{B}^\top$}, fill=red!20, greatgrandchild
                                		[{$l = n + r$}, fill=red!10, referenceblock]
                            	]
			]
			%-------------------------------------------------------------
                    	[2. Random Matrix based Hypernet Reconciliation, fill=red!30, grandchild
				[{2-(a). $\psi(\mb{w}) = \left( \sigma \left( (\mb{w} \mb{P}) \mb{Q}^\top \right) \mb{S} \right) \mb{T}^\top$}, fill=red!20, greatgrandchild
                                		[{$l$ manual setup}, fill=red!10, referenceblock]
                            	]
			]
		]                    
		[Remainder Functions, for tree={fill=blue!45, child}
                        [1. \sout{Expansion Remainder}, fill=blue!30, grandchild
				[{1-(a). $\msout { \pi(\mb{x} | \mb{w}') = \left\langle \kappa'(\mb{x}), \psi'(\mb{w}') \right\rangle + \pi'(\mb{x})}$}, fill=blue!20, greatgrandchild
                                		[\sout{requires parameter}, fill=blue!10, referenceblock]
                            	]
			]
                ]
            ]
            \end{forest}
    \end{center}
    \caption{An overview of the updated data expansion, parameter reconciliation, and remainder functions implemented in the {\toolkit} toolkit for constructing the {\our} model architecture. The crossline added to the ``Expansion Remainder'' denotes the function has been deleted from the toolkit.}\label{fig:updated_component_function}
\end{figure*}
%\vspace{2em}
%\hrule
%------------------------------------------------------------------------------------



==> sections/sec_improvement.tex <==
%--------------------------------------------------------------------------
\section{Advancing Existing Backbone Models with {\our}}\label{sec:backbone_improvement}

In this section, we will delve into a discussion of these weaknesses from the perspective of {\our} of the existing backbone models based on their unified representations. This analysis may not only illuminate new ideas for enhancing existing models but also inspire the proposal of novel models to supersede them. By examining these established architectures through the lens of our unified framework, we aim to provide fresh insights that could drive innovation in model design and performance optimization.

\subsection{Weakness of CNN}

The overall feeling about CNN is that it is an old-style model using many ad hoc architecture designs

stride and pooling is more like a compromise to the computational resources so as to sample useful features

cannot maintain the rotational invariance

Moreover, patches with the cylinder shape may maintain the rotational-invariance (with rotational axis perpendicular to circular surface), and patches with the sphere shape is rotational-invariance along all the rotational axis.

However, the padding based parameter reconciliatioin will break such a good property... 

\subsubsection{Interdependency Modeling}

it uses redundant expansion to model the regional interdependency, lacks the long-distance feature and cross-instance interdependency modeling ability

\subsubsection{Data Expansion}

identity data expansion

\subsubsection{Parameter Reconciliation Function}

duplicated padding based reconciliation

\subsubsection{Remainder Function}

The vanilla version uses zero remainder, and the recent ResNet uses the linear remainder.


\subsection{Weakness with RNN}

For the above Equation~(\ref{equ:rnn_hidden_state}), we rewrite it and also compare it with another similar recurrent state updating operator as follows. The main differences between these above two formula lie in the inputs to updating operators:

\begin{minipage}{0.45\textwidth}
\begin{equation}
\begin{cases}
\ \mb{h}_1' &= \sigma \left( \mb{h}_{0} \mb{U} + \mb{h}_1 \right), \\
\ \mb{h}_2' &= \sigma \left( \mb{h}_{1}' \mb{U} + \mb{h}_2 \right), \\
\ \mb{h}_3' &= \sigma \left( \mb{h}_{2}' \mb{U} + \mb{h}_3 \right), \\
\ \cdots & \cdots \\
\ \mb{h}_b' &= \sigma \left( \mb{h}_{b-1}' \mb{U} + \mb{h}_b \right);
\end{cases}
\end{equation}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\begin{equation}
\begin{cases}
\ \mb{h}_1' &= \sigma \left( \mb{h}_{0} \mb{U} + \mb{h}_1 \right), \\
\ \mb{h}_2' &= \sigma \left( \mb{h}_{1} \mb{U} + \mb{h}_2 \right), \\
\ \mb{h}_3' &= \sigma \left( \mb{h}_{2} \mb{U} + \mb{h}_3 \right), \\
\ \cdots & \cdots \\
\ \mb{h}_b' &= \sigma \left( \mb{h}_{b-1} \mb{U} + \mb{h}_b \right).
\end{cases}
\end{equation}
\end{minipage}

For the one at the left-hand-side, identical as the RNN model discussed above, when updating the state vector $\mb{h}_i'$ (for $\forall i \in \{1, 2, \cdots, b\}$), it will accept $h_{i-1}'$ and $h_i$ as the inputs, where $h_{i-1}'$ was recursively updated with $h_{i-2}'$ and so forth. In other words, $\mb{h}_i'$ can access all the input information before it via $h_{i-1}'$. However, such sequential dependence among the state vectors $\mb{h}_1', \mb{h}_2', \cdots, \mb{h}_b'$ actually prevents the concurrent updating of the inputs' states, we have to compute $\mb{h}_1'$ first, and then $\mb{h}_2'$, and so forth, which can be slow for longer sequence inputs.

However, for the operator at the right-hand-side, when updating the state vector $\mb{h}_i'$, its inputs are $h_{i-1}$ and $h_i$ instead, where $h_{i-1}$ was defined based $\mb{x}_{i-1}$ only. Therefore, $\mb{h}_i'$ can only access information that is 1-hop away from it. To enable $\mb{h}_i'$ access all the inputs' information before it, we may need to either apply the operator at least $i-1$ times on the states' vectors or propose other approaches for modeling such multi-hop dependence relationships. Moreover, the advantages of the right operator is that we can rewrite it into a batch for concurrent updating, which can be represented as follows:

\begin{equation}
\mb{H} = \sigma \left( \mb{A} \mb{H} \mb{U} + \mb{H} \right),
\end{equation}

where 

\begin{equation}
\mb{A} = \begin{bmatrix}
0 & 0 & 0 & \cdots & 0 & 0 \\
1 & 0 & 0 & \cdots & 0 & 0 \\
0 & 1 & 0 & \cdots & 0 & 0 \\
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
0 & 0 & 0 & \cdots & 1 & 0 \\
\end{bmatrix} \in \mathbbm{R}^{(b+1) \times (b+1)} \text{ , and } \mb{H} = [\mb{h}_0, \mb{h}_1, \mb{h}_2, \cdots, \mb{h}_b]^\top \in \mathbbm{R}^{(b+1) \times d_h}.
\end{equation}

The matrix $\mb{H}$ denotes the input sequence batch. For simplicity, we also include the dummy input vector $\mb{h}_0$ into the batch as well. The matrix $\mb{A}$ actually denotes the chain based structural interdependence matrix as introduced in the previous Section~\ref{subsubsec:chain_interdependence_function}. A note we need mention here is that the chain based structural interdependence matrix defined in the previous section is for the attributes, which may look different from the above matrix defined for the instances. Furthermore, by replacing the above matrix $\mb{A}$ with the multi-hop chain based structure interdependence functions introduced in the previous Section~\ref{subsubsec:multihop_chain_interdependence_function}, we will be capable to update the state vectors with information all before the current inputs, which is similar to the RNN model discussed above.


\subsection{Weakness with GNN}


\subsection{Weakness with Transformer}


\subsection{Surpassing These Backbone Models with {\our}}




==> tables/language_classification_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:language_classification_benchmark_results}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{\textbf{Language Classification Datasets}}  \\
        \cline{2-4}
         & \textbf{IMDB} & \textbf{AGNews} & \textbf{SST2}  \\
        \hline
        \hline
        \makecell{MLP} 
        & \makecell{$8.85 \times 10^{-1}$} 
        & \makecell{\boldmath $9.21 \times 10^{-1}$} 
        & \makecell{ $8.05 \times 10^{-1}$} \\
        \hline
        \hline
        \makecell{Previous {\old} \cite{zhang2024rpnreconciledpolynomialnetwork}} 
        & \makecell{$8.86 \times 10^{-1}$} 
        & \makecell{$9.19 \times 10^{-1}$} 
        & \makecell{$8.07 \times 10^{-1}$}\\
        \hline
%        \hline
%        \makecell{RNN} 
%        & 
%        & 
%        & \\
%        \hline
%        \hline
%        \makecell{Transformer} 
%        & 
%        & 
%        & \\
%        \hline
        \hline
        \makecell{{\our}\\ (chain interdependence)}
        & \makecell{\boldmath $8.90 \times 10^{-1}$} 
        & \makecell{\boldmath $9.21 \times 10^{-1}$} 
        & \makecell{\boldmath $8.17 \times 10^{-1}$} \\
        \hline
%        \hline
%        \makecell{{\our}\\ (bilinear)}
%        & 
%        & 
%        & \\
%        \hline
    \end{tabular}
\end{table}

%MNIST: [784, 64, 64, 10]	taylor, identity, zero	1 head per layer	[2, 2, 2]	2e-3, wd 2e-4, gamma 0.9	9875
%\makecell{{\our}} & \makecell{\boldmath $9.86 \times 10^{-1}$ \\ \boldmath $\pm$  $8.70 \times 10^{-4}$ \\ {- - - - - - - - - - - -} \\ $[$784, 64, 64, 10$]$ \\ (taylor, identity, zero)} & \makecell{ $5.61 \times 10^{-1}$ \\  $\pm$  $1.66 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$3072, 512, 256, 10$]$ \\ (identity, masking, zero)} & \makecell{\boldmath$8.86 \times 10^{-1}$  \\ \boldmath$\pm$ $4.59 \times 10^{-4}$ \\ {- - - - - - - - - - - -} \\ $[$26964, 128, 32, 2$]$ \\ (identity, lorr, zero)} & \makecell{$9.19 \times 10^{-1}$  \\ $\pm$ $2.55 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$25985, 128, 4$]$\\ (identity, lorr, zero)} & \makecell{\boldmath $8.07 \times 10^{-1}$  \\ \boldmath $\pm$ $1.72 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$10325, 128, 32, 2$]$\\ (identity, lorr, zero)}\\

==> tables/language_dataset_statistics.tex <==
\begin{table}[t]
\centering
\small
\caption{TBD}
\label{tab:language_dataset_statistics}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{Language Classification Datasets}} & \multicolumn{3}{c|}{\textbf{Language Generation Datasets}} \\ \cline{2-7}
                          & \textbf{IMDB} & \textbf{AGNews} & \textbf{SST2} & \textbf{TBD} & \textbf{TBD} & \textbf{TBD} \\ \hline\hline
Train \#                     & 25,000  & 120,000  & 67,349 & & &  \\ \hline
Test \#                     & 25,000  & 7,600  & 872  & & &  \\ \hline
Input Dim.                     & TBD  & TBD  & TBD & & &   \\ \hline
Output Dim.                     & 2  & 4  & 2  & & &  \\ \hline
\end{tabular}
\end{table}

%& \textbf{ImageNet} 
%& 1,281,167  
%& 50,000  
%& 224 $\times$ 224 $\times$ 3  
%& 1,000  

==> tables/language_generation_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:language_generation_benchmark_results}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{\textbf{Language Generation Datasets}}  \\
        \cline{2-4}
        & \textbf{TBD} & \textbf{TBD} & \textbf{TBD}  \\
        \hline
        \hline
        \makecell{RNN} 
        & 
        & 
        & \\
        \hline
        \hline
        \makecell{Transformer} 
        & 
        & 
        & \\
        \hline
        \hline
        \makecell{{\our}\\ (chain)}
        & 
        & 
        & \\
        \hline
        \hline
        \makecell{{\our}\\ (bilinear)}
        & 
        & 
        & \\
        \hline
    \end{tabular}
\end{table}


==> tables/vision_classification_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:vision_classification_benchmark_results}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c|}{\textbf{Image Datasets}}  \\
        \cline{2-4}
         & \textbf{MNIST} & \textbf{CIFAR10} & \textbf{IMAGENET} \\
        \hline
         \hline
	\makecell{MLP} 
	& \makecell{ $9.82 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ $[$784, 512, 256, 10$]$} 
	& \makecell{ $5.63 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ $[$784, 512, 256, 10$]$} 
	&\\
        \hline
        \hline
        \makecell{Previous {\old} \cite{zhang2024rpnreconciledpolynomialnetwork}\\ {(zero remainder)}} 
        & \makecell{ $9.86 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ $[$784, 64, 64, 10$]$ } 
        & \makecell{ $5.61 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ $[$3072, 512, 256, 10$]$ } 
        & \\
        \hline
%        \hline
%        \makecell{CNN} 
%        & \makecell{ $9.64 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ Channel: $[$1, 24, 48, 64$]$ \\ Dim: $[$784, 256, 10$]$ } 
%        & \makecell{ $8.47 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ Channel: $[$3, 128, 128, 256, 256$]$ \\ Dim: $[$16384, 1024, 512, 10$]$ } 
%        & \\
%        \hline
        \hline
        \makecell{{\our}\\ {(grid interdependence}\\ {cylinder patch)}} 
        & \makecell{\boldmath $9.98 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ Channel: $[$1, 24, 48, 64$]$ \\ Dim: $[$784, 256, 10$]$ } 
        & \makecell{\boldmath $8.52 \times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - - -} \\ Channel: $[$3, 128, 128, 256, 256$]$ \\ Dim: $[$16384, 1024, 512, 10$]$ } 
        & \\
        \hline
    \end{tabular}
\end{table}

%MNIST: [784, 64, 64, 10]	taylor, identity, zero	1 head per layer	[2, 2, 2]	2e-3, wd 2e-4, gamma 0.9	9875
%\makecell{{\our}} & \makecell{\boldmath $9.86 \times 10^{-1}$ \\ \boldmath $\pm$  $8.70 \times 10^{-4}$ \\ {- - - - - - - - - - - -} \\ $[$784, 64, 64, 10$]$ \\ (taylor, identity, zero)} & \makecell{ $5.61 \times 10^{-1}$ \\  $\pm$  $1.66 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$3072, 512, 256, 10$]$ \\ (identity, masking, zero)} & \makecell{\boldmath$8.86 \times 10^{-1}$  \\ \boldmath$\pm$ $4.59 \times 10^{-4}$ \\ {- - - - - - - - - - - -} \\ $[$26964, 128, 32, 2$]$ \\ (identity, lorr, zero)} & \makecell{$9.19 \times 10^{-1}$  \\ $\pm$ $2.55 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$25985, 128, 4$]$\\ (identity, lorr, zero)} & \makecell{\boldmath $8.07 \times 10^{-1}$  \\ \boldmath $\pm$ $1.72 \times 10^{-3}$ \\ {- - - - - - - - - - - -} \\ $[$10325, 128, 32, 2$]$\\ (identity, lorr, zero)}\\

==> tables/vision_compression_function_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:vision_compression_function_result}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{\makecell{\textbf{Compression Patch}\\ \textbf{Parameters}}} & \multicolumn{3}{c|}{\textbf{Compression Layer Number}}  \\
        \cline{2-4}
         & \makecell{\textbf{1 Compression Layer}} 
         & \makecell{\textbf{2 Compression Layers}} 
         & \makecell{\textbf{4 Compression Layers}} \\
         \hline
         \hline
	\makecell{\textbf{Compression Patch}\\ \textbf{Center Distance}\\ $p_r = 1$\\ $cd_h=2$\\ $cd_w=2$}
	& \makecell{ accuracy: $8.15\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [16, 16, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 74,064,778} 
	& \makecell{ accuracy: $8.52\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [8, 8, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 23,339,914} 
	& \makecell{ accuracy: $8.29\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [2, 2, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 7,402,378}  \\
        \hline
        \hline
	\makecell{\textbf{Compression Patch}\\ \textbf{Center Distance}\\ $p_r = 2$\\ $cd_h=2$\\ $cd_w=2$}
	& \makecell{ accuracy: $8.18\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [16, 16, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 74,064,778} 
	& \makecell{ accuracy: $8.51\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [8, 8, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 23,339,914} 
	& \makecell{ accuracy: $8.33\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [2, 2, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 7,402,378}  \\
        \hline
        \hline
	\makecell{\textbf{Compression Patch}\\ \textbf{Center Distance}\\ $p_r = 4$\\ $cd_h=2$\\ $cd_w=2$}
	& \makecell{ accuracy: $8.17\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [16, 16, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 74,064,778} 
	& \makecell{ accuracy: $8.48\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [8, 8, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 23,339,914} 
	& \makecell{ accuracy: $8.32\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [2, 2, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 7,402,378}  \\
        \hline
        \hline
	\makecell{\textbf{Compression Patch}\\ \textbf{Center Distance}\\ $p_r = 4$\\ (\text{half after pooling})\\ $cd_h=2$\\ $cd_w=2$}
	& \makecell{ accuracy: $8.18\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [16, 16, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 74,064,778} 
	& \makecell{ accuracy: $8.51\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [8, 8, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 23,339,914} 
	& \makecell{ accuracy: $8.35\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  shape: [2, 2, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 7,402,378}  \\
        \hline
    \end{tabular}
\end{table}


==> tables/vision_cuboid_patch_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:cuboid_patch_results}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multirow{6}{*}{\makecell{\textbf{Packing}\\ \textbf{Strategies}}} & \multicolumn{4}{c|}{\textbf{Cuboid Patch Shapes}}  \\
        \cline{2-5}
         & \makecell{\textbf{Cuboid Shape 1}\\ $p_h=p_h'=1$\\ $p_w=p_w'=1$\\ $p_d=p_d'=0$} 
         & \makecell{\textbf{Cuboid Shape 2}\\ $p_h=p_h'=2$,\\ $p_w=p_w'=2$\\ $p_d=p_d'=0$} 
         & \makecell{\textbf{Cuboid Shape 3}\\ $p_h=p_h'=3$,\\ $p_w=p_w'=3$\\ $p_d=p_d'=0$}
         & \makecell{\textbf{Cuboid Shape 4}\\ $p_h=p_h'=4$,\\ $p_w=p_w'=4$\\ $p_d=p_d'=0$}\\
         \hline
         \hline
	\makecell{\textbf{Sparse Square}\\ $cd_h=3p_h$\\ $cd_w = 3p_w$\\ $cd_d = 3p_d$}
	& \makecell{ accuracy: $6.20\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 2 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,223,690} 
        & \makecell{ accuracy: $4.39\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,085,962} 
        & \makecell{ accuracy: $5.92\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,485,834}
        & \makecell{ accuracy: $5.61\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,021,514}  \\
        \hline
        \hline
        \makecell{\textbf{Complete Square}\\ $cd_h=2p_h$\\ $cd_w = 2p_w$\\ $cd_d = 2p_d$}
        & \makecell{ accuracy: $7.33\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,819,978} 
        & \makecell{ accuracy: $5.90\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,089,930} 
        & \makecell{ accuracy: $5.55\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,488,394}
        & \makecell{ accuracy: $6.04\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,022,410}  \\
        \hline
        \hline
        \makecell{\textbf{Dense Square}\\ $cd_h=p_h$\\ $cd_w = p_w$\\ $cd_d = p_d$}
        & \makecell{ accuracy: $7.56\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,161,738} 
        & \makecell{ accuracy: $7.37\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 3,088,266} 
        & \makecell{ accuracy: $6.21\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 2 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,894,410}  
        & \makecell{ accuracy: $6.32\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,028,938}  \\        
        \hline
        \hline
        \makecell{\textbf{Densest Packing}\\ $cd_h=1$\\ $cd_w =1$\\ $cd_d = 1$}
        & \makecell{ accuracy: $7.56\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,161,738} 
        & \makecell{ accuracy: $7.69\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,430,026} 
        & \makecell{ accuracy: $7.74\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,832,458}
        & \makecell{ accuracy: $7.71\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 136,369,034}  \\
        \hline
    \end{tabular}
\end{table}


==> tables/vision_cylinder_patch_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:cylinder_patch_results}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multirow{5}{*}{\makecell{\textbf{Packing}\\ \textbf{Strategies}}} & \multicolumn{4}{c|}{\textbf{Cylinder Patch Shapes}}  \\
        \cline{2-5}
         & \makecell{\textbf{Cylinder Shape 1}\\ $p_r=1$,\\ $p_d=p_d'=0$} 
         & \makecell{\textbf{Cylinder Shape 2}\\ $p_r=2$,\\ $p_d=p_d'=0$} 
         & \makecell{\textbf{Cylinder Shape 3}\\ $p_r=3$,\\ $p_d=p_d'=0$}
         & \makecell{\textbf{Cylinder Shape 4}\\ $p_r=4$,\\ $p_d=p_d'=0$}\\
         \hline
         \hline
	\makecell{\textbf{Sparse Square}\\ $cd_h=2p_r$\\ $cd_w = 2p_r$\\ $cd_d = 2p_d$}
	& \makecell{ accuracy: $6.85\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,752,906} 
        & \makecell{ accuracy: $5.44\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 888,714} 
        & \makecell{ accuracy: $4.63\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,153,034}  
        & \makecell{ accuracy: $5.89\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,485,834}  \\
        \hline
        \hline
        \makecell{\textbf{Complete Square}\\ $cd_h=\sqrt{2}p_r$\\ $cd_w = \sqrt{2}p_r$\\ $cd_d = 2p_d$}
        & \makecell{ accuracy: $7.27\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,094,666} 
        & \makecell{ accuracy: $7.36\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,887,050} 
        & \makecell{ accuracy: $6.02\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,157,002}
        & \makecell{ accuracy: $6.33\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,490,442}  \\
        \hline
        \hline
        \makecell{\textbf{Sparse Hexagonal}\\ $cd_h=\sqrt{3}p_r$\\ $cd_w = {2}p_r$\\ $cd_d = 2p_d$}
        & \makecell{ accuracy: $7.22\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 17,490,314} 
        & \makecell{ accuracy: $5.94\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,023,370} 
        & \makecell{ accuracy: $5.62\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,153,930}
        & \makecell{ accuracy: $5.64\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,486,858}  \\        
        \hline
        \hline
        \makecell{\textbf{Complete Hexagonal}\\ $cd_h=\frac{3}{2}p_r$\\ $cd_w = \sqrt{3}p_r$\\ $cd_d = 2p_d$}
        & \makecell{ accuracy: $7.27\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,094,666} 
        & \makecell{ accuracy: $6.28\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 2 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,290,762} 
        & \makecell{ accuracy: $6.05\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,155,978}
        & \makecell{ accuracy: $5.56\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $1 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,488,394}  \\
        \hline
        \hline
        \makecell{\textbf{Dense Hexagonal}\\ $cd_h=\frac{\sqrt{6}}{2}p_r$\\ $cd_w = \sqrt{2}p_r$\\ $cd_d = p_d$}
        & \makecell{ accuracy: $7.27\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,094,666} 
        & \makecell{ accuracy: $7.36\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,887,050} 
        & \makecell{ accuracy: $6.13\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,291,658}
        & \makecell{ accuracy: $6.28\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,491,338}  \\
        \hline
        \hline
        \makecell{\textbf{Denser Hexagonal}\\ $cd_h=\frac{\sqrt{3}}{2}p_r$\\ $cd_w = p_r$\\ $cd_d = p_d$}
        & \makecell{ accuracy: $7.26\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,094,666} 
        & \makecell{ accuracy: $7.51\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 4 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 17,624,458} 
        & \makecell{ accuracy: $6.78\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $4 \times 2 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 2,092,426}
        & \makecell{ accuracy: $6.23\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $2 \times 1 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 1,627,018}  \\
        \hline
        \hline
        \makecell{\textbf{Densest Packing}\\ $cd_h=1$\\ $cd_w =1$\\ $cd_d = 1$}
        & \makecell{ accuracy: $7.27\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,094,666} 
        & \makecell{ accuracy: $7.61\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,228,810} 
        & \makecell{ accuracy: $7.76\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,497,098}
        & \makecell{ accuracy: $7.80\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\ shape: $32 \times 32 \times 128$ \\ {- - - - - - - - - - - - - - - - -} \\ para. num: 135,832,458}  \\
        \hline
    \end{tabular}
\end{table}


==> tables/vision_depth_width_results.tex <==
\begin{table}[t]
    \caption{TBD}
    \label{tab:vision_depth_width_result}
    \small
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\makecell{\textbf{Channel}\\ \textbf{Numbers}}} & \multicolumn{4}{c|}{\textbf{Model Depth (Grid based Structural Interdependence Layers)}}  \\
        \cline{2-5}
         & \makecell{\textbf{1 Layer}} 
         & \makecell{\textbf{2 Layers}} 
         & \makecell{\textbf{3 Layers}} 
         & \makecell{\textbf{4 Layers}} \\
         \hline
         \hline
	\makecell{\textbf{64}\\ \textbf{Channels}}
	& \makecell{ accuracy: $7.51\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 67,714,762} 
	& \makecell{ accuracy: $7.65\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64, 64] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 67,981,002} 
	& \makecell{ accuracy: $7.82\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64, 64, 64] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 68,247,242} 
	& \makecell{ accuracy: $7.92\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64, 64, 64, 64] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 68,513,482}  \\
        \hline
        \hline
        \makecell{\textbf{128}\\ \textbf{Channels}}
        & \makecell{ accuracy: $7.59\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 134,898,570} 
	& \makecell{ accuracy: $7.79\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128, 128] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 135,832,458} 
	& \makecell{ accuracy: $8.03\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128, 128, 128] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 136,766,346} 
	& \makecell{ accuracy: $8.18\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128, 128, 128, 128] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 137,700,234}  \\
        \hline
        \hline
        \makecell{\textbf{256}\\ \textbf{Channels}}
        & \makecell{ accuracy: $7.63\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 269,266,186} 
	& \makecell{ accuracy: $7.81\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 256, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 272,739,594} 
	& \makecell{ accuracy: $8.09\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 256, 256, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 276,213,002} 
	& \makecell{ accuracy: $8.23\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 256, 256, 256, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 279,686,410}  \\        
        \hline
        \hline
        \makecell{\textbf{Increasing}\\ \textbf{Channels}}
        & \makecell{ accuracy: $7.51\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 67,714,762} 
	& \makecell{ accuracy: $7.78\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 64, 128] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 135,356,106} 
	& \makecell{ accuracy: $8.06\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128, 128, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 271,917,962} 
	& \makecell{ accuracy: $8.20\times 10^{-1}$ \\ {- - - - - - - - - - - - - - - - -} \\  channel: [3, 128, 128, 256, 256] \\  {- - - - - - - - - - - - - - - - -} \\ para. num: 275,391,370}  \\
        \hline
    \end{tabular}
\end{table}

